A Fully Polynomial Time Approximation Scheme for Constrained MDPs and Stochastic Shortest Path under Local Transitions

The fixed-horizon constrained Markov Decision Process (C-MDP) is a well-known model for planning in stochastic environments under operating constraints. Chance-Constrained MDP (CC-MDP) is a variant that allows bounding the probability of constraint violation, which is desired in many safety-critical applications. CC-MDP can also model a class of MDPs, called Stochastic Shortest Path (SSP), under dead-ends, where there is a trade-off between the probability-to-goal and cost-to-goal. This work studies the structure of (C)C-MDP, particularly an important variant that involves local transition. In this variant, the state reachability exhibits a certain degree of locality and independence from the remaining states. More precisely, the number of states, at a given time, that share some reachable future states is always constant. (C)C-MDP under local transition is NP-Hard even for a planning horizon of two. In this work, we propose a fully polynomial-time approximation scheme for (C)C-MDP that computes (near) optimal deterministic policies. Such an algorithm is among the best approximation algorithm attainable in theory and gives insights into the approximability of constrained MDP and its variants.

==> append.tex <==
\section*{Appendix}

\subsection*{Proof of Lemma \ref{lem:minks}}
% \begin{lemma}\label{lem:minks}
% Algorithm {\tt Dyn-MinKS} obtains a solution $\Bell = (\ell^1,..., \ell^{|\cN|})$ that  satisfies
% \begin{align}
% &\sum_{i \in \cN}  w_{i,\ell^{i}} \le \sum_{i \in \cN}  w_{i,\ell^{i*}}, &\text{ and }&
% &\sum_{i \in \cN}  v_{i,\ell^{i}} \ge \sum_{i \in \cN}  v_{i,\ell^{i*}} -  |\cN| R_k,
% \end{align}
% where $\Bell^*$ is an optimal solution.
% \end{lemma}
\begin{proof}
Define $\overline v_{i, \ell^i} := \lfloor v_{i, \ell^i}/R_k \rfloor R_k$ as in Line~\ref{alg:discdem} of {\tt Dyn-MinKS} (also define $\overline v_{i,\ell^{i*}} := \lfloor v_{i, \ell^{i*}}/R_k \rfloor R_k$).   Since the algorithm discretizes values (Line~\ref{alg:discdem}), and  the largest element of $\cR$ is an upper bound on $\sum_{i \in \cN}  \overline v_{i,\ell^{i*}} $  (by the definition of $\cR$ in Eq.~\raf{eq:defR}), then any discretized optimal total values are considered in the table. The algorithm maintains a table {\tt TB}$(i,\rho)$ of minimum total item weights up to user $i$ that satisfies a total value of at least $\rho$. Therefore in steps~\ref{alg:fetch1}-\ref{alg:fetch2}, the algorithm obtains a minimum $\rho \ge D$ that accrues the least total weight, hence $\sum_{i \in \cN}  w_{i,\ell^{i}} \le \sum_{i \in \cN}  w_{i,\ell^{i*}}$. By the feasibility of optimal solutions $\sum_{i \in \cN} \overline v_{i,\ell^{i*}} \ge D$, and since $\rho$ is the least element that satisfies $\rho \ge D$,  we have
\begin{equation} \label{eq:minks-d}
\sum_{i \in \cN} \overline v_{i,\ell^{i}} \ge \sum_{i \in \cN} \overline v_{i,\ell^{i*}}.
\end{equation}
Thus, by Eq.~\raf{eq:minks-d} and rounding values down (Line~\ref{alg:discdem} of {\tt Dyn-MinKS}), 
\begin{align*}
\sum_{i \in \cN}  v_{i,\ell^{i}} &\ge \sum_{i \in \cN} \overline v_{i,\ell^{i}} \ge \sum_{i \in \cN} \overline v_{i,\ell^{i*}} \ge \sum_{i \in \cN} (v_{i,\ell^{i*}} - R_k) 
&= \sum_{i \in \cN} v_{i,\ell^{i*}} -  |\cN| R_k ,
\end{align*}
which completes the proof.


\end{proof}

\subsection*{Proof of Corollary~\ref{thm:fptas2}}
% \begin{corollary} \label{thm:fptas2}
% 	Algorithm {\tt dis-DynSSP} is an FPTAS for (C)C-SSP under disjoint transition assumption.
% \end{corollary}
\begin{proof}
First, observe that the algorithm maintains a dynamic programming table with minimum execution risk. Lines~\ref{alg:f1} of subroutine {\tt Fetch-Policy} ensures that a feasible solution with such property is constructed. The algorithm  runs in polynomial time as the sizes of $\cL_k$ and $\cR_k$ are polynomial. %,  $O(\tfrac{h^{2} \ln h}{\epsilon^2}|\cA| |\cS|)$.
By Lemma~\ref{lem:dis} and Lemma~\ref{lem:opt2}, expanding for $s_0$, and by the definition of $L_k$ and $R_k$, we obtain
	\begin{align}
		\overline v_\pi(s_0)  &\ge \overline v_{\pi^*}(s_0)   - 2 \sum_{k'=0}^{h-1} L_{k'} \\
        &\ge  v_{\pi^*}(s_0) - \sum_{k'=0}^{h-1}L_{k'}  - 2 \sum_{k'=k}^{h-1} L_{k'}\\
        & = v_{\pi^*}(s_0) - 3 \sum_{k=0}^{h-1} \frac{\epsilon U_{\max}}{3(h-k)(\ln h + 1)} \\
		&= v_{\pi^*}(s_0) - \frac{\epsilon U_{\max}}{\ln h + 1} \sum_{k=0}^{h-1} \frac{1}{(h-k)} \notag \\
        &\ge v_{\pi^*}(s_0) - \frac{\epsilon U_{\max}}{\ln h + 1} (\ln h + 1)  \label{eq:harr2}\\
		%h \frac{\epsilon U_{\max}}{h}\\
		&\ge (1-\epsilon)\cdot v_{\pi^*}(s_0), \
	\end{align}
where Eq.~\raf{eq:harr2} follows by using an upper bound on the harmonic series, $\sum_{n=1}^k \tfrac{1}{n} \le \ln k + 1$. Therefore,
\begin{align}
	v_\pi(s_0) \ge  \overline  v_{\pi}(s_0) \ge  (1-\epsilon) v_{\pi^*}(s_0),
\end{align}
which completes the proof.

\end{proof}

==> hard.tex <==
\vspace{-13pt}
\section{Hardness of (C)C-SSP}
\vspace{-10pt}
In this work, we address a research gap concerning the approximability of (C)C-SSP beyond the NP-hardness result \cite{khonji2021dual} (which shows the hardness for a restrictive case of horizon two, under which both local and limited transition assumptions hold). Given the problem is NP-hard, if we require an algorithm that runs in polynomial time for all inputs, the best hope is FPTAS. 
Suppose we allow non-negative parameters, such as rewards or costs (i.e., constrained (C)C-MDP setting). One can show that no $\alpha$-approximation algorithm exists unless P=NP, where $\alpha$ is any non-negative number with a polynomial number of bits. (This result can be proved using a gadget that utilizes an $\alpha$-approximation algorithm for C-MDP to solve any instance of the NP-hard subset sum problem. A similar proof idea is found in Theorem 4.1 in \cite{chau2016truthful}, applied to a variant of the Knapsack problem.) 
\iffalse
The local transition assumption has a central role in problem difficulty. The assumption leads to a reduction to a multi-dimensional knapsack instance with a constant number of constraints (illustrated in Alg.~\ref{alg:update3}, Sec.~\ref{sec:fptas}). If we drop the local transition assumption, the number of constraints can grow to a polynomial (a problem called {\em packing integer program}). Thus, with a polynomial number of constraints, the reduced multi-dimensional knapsack cannot be (approximately) solved in polynomial time, and the FPTAS breaks down.
In fact, one can show that any packing integer program can be reduced to (C)C-SSP (without local transition assumption) and prove that no ($\psi^{1/2 - \epsilon}$)-approximation exists for (C)C-SSP unless P=NP (based on existing hardness result for packing integer programming \cite{chekuri2004multidimensional}). 
\fi


